AI for Global Climate Cooperation: Modeling Global Climate Negotiations, Agreements, and Long-Term Cooperation in RICE-N

Comprehensive global cooperation is essential to limit global temperature increases while continuing economic development, e.g., reducing severe inequality or achieving long-term economic growth. Achieving long-term cooperation on climate change mitigation with n strategic agents poses a complex game-theoretic problem. For example, agents may negotiate and reach climate agreements, but there is no central authority to enforce adherence to those agreements. Hence, it is critical to design negotiation and agreement frameworks that foster cooperation, allow all agents to meet their individual policy objectives, and incentivize long-term adherence. This is an interdisciplinary challenge that calls for collaboration between researchers in machine learning, economics, climate science, law, policy, ethics, and other fields. In particular, we argue that machine learning is a critical tool to address the complexity of this domain. To facilitate this research, here we introduce RICE-N, a multi-region integrated assessment model that simulates the global climate and economy, and which can be used to design and evaluate the strategic outcomes for different negotiation and agreement frameworks. We also describe how to use multi-agent reinforcement learning to train rational agents using RICE-N. This framework underpinsAI for Global Climate Cooperation, a working group collaboration and competition on climate negotiation and agreement design. Here, we invite the scientific community to design and evaluate their solutions using RICE-N, machine learning, economic intuition, and other domain knowledge. More information can be found on www.ai4climatecoop.org.

==> src_AAAI/env_model.tex <==
%!TEX root = main.tex

% %\newcommand\argmax{}[]{\arg\max}
% \begin{itemize}
%     \item RICE model
    
%     \item Calibration in brief and sources. Include details in Appendix
% \end{itemize}

\subsection{The RICE model}

% The RICE (Regional Dynamic General-Equilibrium) model \cite{rice} is implemented based on the DICE model. Among many DICE model implementations, we followed \cite{DBLP:journals/corr/abs-1812-08066}. Basically, each region has its own parameters and developing pattern because of different populations, technology development, capital accumulation etc. However, they all emit $CO_2$ and suffer the same temperature raising issue. 



% Overview
\begin{equation}
 \begin{aligned} T(i+1) &=\Phi_{T} T(i)+B_{T}\left(F_{2 \times} \log _{2}\left(\frac{M_{\mathrm{AT}}(i)}{M_{\mathrm{AT}, 1750}}\right)+F_{\mathrm{EX}}(i)\right) \\ M(i+1) &=\Phi_{M} M(i)+B_{M}\left(\sigma(i)(1-\mu(i)) A(i) K(i)^{\gamma} L(i)^{1-\gamma}+E_{\mathrm{Land}}(i)\right), \\ K(i+1) &=\Phi_{K} K(i)+\Delta\left(1-a_{1} T_{\mathrm{AT}}(i) - a_{2} T_{\mathrm{AT}}(i)^{2} \right)\left(1-\theta_{1}(i) \mu(i)^{\theta_{2}}\right) A(i) K(i)^{\gamma} L(i)^{1-\gamma} s(i), \\ L(i+1) &=L(i)\left(\frac{1+L_{a}}{1+L(i)}\right)^{\ell_{g}}, \\ A(i+1) &=(\exp\eta+g_{A} \exp \left(-\delta_{A} \Delta(i-1)\right))A(i), \\ \sigma(i+1) &=\sigma(i) \exp \left(-g_{\sigma}\left(1-\delta_{\sigma}\right)^{\Delta(i-1)} \Delta\right), \end{aligned}
\end{equation}

There are predetermined parameters in the above dynamics. There are also some parameters whose values are not defined. To determine these values, we use the known historical time series data to estimate them. This process is called as \textbf{parameter caliberation}.
\subsubsection{Social Economics Dynamics}
\paragraph{Population}
\begin{equation}
\label{pop}
L(i+1) =L(i)\left(\frac{1+L_{a}}{1+L(i)}\right)^{\ell_{g}}
\end{equation}
Explanation: There are two parameters $L_a$ and $l_g$. If we take the $\lim$ operator on both sides of the equations and denote $L_{\infty}:=\lim_{n\rightarrow \infty} L(n)$, we will have
\begin{equation}
 \begin{aligned}
 L_{\infty} &= L_{\infty} (\frac{1+L_a}{1+L_{\infty}})^{l_g}\\
 1 &= (\frac{1+L_a}{1+L_{\infty}})^{l_g}
 \end{aligned}
\end{equation}
As long as $l_g$ is not zero, $L_{\infty} = L_{a}$. Thus, $L_a$ is a predetermined parameter which is expected to be the convergence population. We used the data from the world bank. Assuming $L(n)$ is monotonically increasing or decreasing, the absolute value of $l_g$ represents how fast $L(n)$ converges to $L_a$.

In the parameter caliberation, the closer this time series is to monotonically increasing or monotonically decreasing, the less difficult it is to adjust the parameters.

In detail, we have the historical population time series $L(n) \quad n\in\{1,2,...,N\}$ is known, we need to find the undefined parameter $l_g$ to estimate future population data.

It is evident that the equation \ref{pop} is equivalent to \begin{equation}\log{L(i+1)} - \log{L(i)} = l_g (\log{(1+L_a)} - \log{(1+L(i))})\end{equation} where $\log{L(i+1)} - \log{L(i)}$ and $\log{(1+L_a)} - \log{(1+L(i))}$ is given. $l_g$ can be estimated by linear regression without intercept.
\paragraph{Technology}
% A_i * (np.exp(0.0033) + g_A * math.exp(-delta_A * Delta * (ii - 1)))
\begin{equation}
A(i+1) =(\exp\eta+g_{A} \exp \left(-\delta_{A} \Delta(i-1)\right))A(i)
\end{equation}

Explanation: There are three parameters: $\eta$, $g_A$ and $\delta_A$. Among then, $\eta$ means the long-term growth of economics which is usually larger than 0 and $g_A$ represents the short-term part of economics growth and $delta_A$ represents the speed of decay of short-term growth factor. $Delta$ is the time difference between steps. We take $\eta$ as $0.33\%$ which is also set by the original DICE paper. A healthy-developing economics should have $g_A > 0$ and $\delta_A > 0$.

In the parameter calibration, we need to estimate both $g_A$ and $\delta_A$ from the existing data $A(n)$.
\begin{equation}
g_{A}^{*}, \delta_{A}^{*} = \arg \max_{g_{A}, \delta_{A}} ||A(i+1) - (\exp\eta+g_{A} \exp \left(-\delta_{A} \Delta(i-1)\right))A(i)||^2
\end{equation}
In practice, we get the solution by numerical optimization algorithms in scipy.

\paragraph{Output Production}
\begin{equation}
    Y(i) = A(i)K(i)^{\gamma}L(i)^{(1-\gamma)}
\end{equation}
We follow the DICE model production function and define the production output multiplication of three factors: the total factor productivity (Technology) $A(i)$, capital $K(i)$ and labor $L(i)$. The capital elasticity $\gamma \in [0,1]$ explains the different contribution level of capital and labor. Please also notice that 
\begin{equation}
    \begin{aligned}
        Y(i) &= (A(i)K(i))^{\gamma}(A(i)L(i))^{(1-\gamma)}\\
        c\cdot Y(i) &= (c\cdot A(i)K(i))^{\gamma}(c\cdot A(i)L(i))^{(1-\gamma)}\quad \forall c\in \mathbb{R}^{+}
        \\ \hspace*{\fill} \\
        c\cdot Y(i) &\neq (c\cdot A(i))(c\cdot K(i))^{\gamma}(c\cdot L(i))^{(1-\gamma)}
    \end{aligned}
\end{equation}
Usually $A(i)K(i)$ is regarded as the effective capital and $A(i)L(i)$ is the effective labor. To sum up the production across different regions, we should sum up the effective capital and effective labor instead of the total factor productivity, capital and labor.

\paragraph{Carbon intensity of economics activity}
\begin{equation}
\begin{aligned}
    E_{\text {Land }}(i)&=E_{L0} \cdot\left(1-\delta_{E L}\right)^{i-1}\\
    \sigma(i)&:=\frac{E(i)-E_{\text {Land }}(i)}{(1-\mu(i)) A(i) K(i)^{\gamma} L(i)^{1-\gamma}}\\
    \sigma(i+1) &=\sigma(i) \exp \left(-g_{\sigma}\left(1-\delta_{\sigma}\right)^{\Delta(i-1)} \Delta\right)
\end{aligned}
\end{equation}
The $E_{\text{land}}(n)$ is the emissions due to land use changes where $E_{L0}$ is the land-use change in the base year and the $\delta_{EL}$ is the speed of decreasing of land use changes between 0 and 1. \\
The $E{n}$ is the total carbon emission and $E{n} - E_{\text{land}}(n)$ explains the carbon emission by economics activities. The $\mu$ in the denominator is a control variable called the abatement ratio which represents the proportion of the economics contributing to reducing carbon emission. Thus, the whole denominator represents the net production and the $\sigma(i)$ is called as the carbon intensity of economics activity.\\
In the dynamic of $\sigma$, we have 2 parameters $g_{\sigma}$ and $\delta_{\sigma}$. $g_{\sigma}$ is the expected to be the decreasing speed of the carbon emission.\\
However, the emission data we collected from the world bank database does not fit for the form of $\sigma$ dynamic assuming by DICE2016. We therefore give up calibrate the parameters $g_{\sigma}$ and $\delta_{\sigma}$ and refer to the parameters given by DICE2016. 

\paragraph{Capital}
\begin{equation}
    \begin{aligned}
    \Phi_{K} &\doteq\left(1-\delta_{K}\right)^{\Delta}\\
    K(i+1) &=\Phi_{K} K(i)+\Delta\left(1-a_{1} T_{\mathrm{AT}}(i) - a_{2} T_{\mathrm{AT}}(i)^{2} \right)\left(1-\theta_{1}(i) \mu(i)^{\theta_{2}}\right) A(i) K(i)^{\gamma} L(i)^{1-\gamma} s(i)
    \end{aligned}
\end{equation}
The evolution of the capital comes from 2 parts. The first part is undepreciated capital inherited from the previous period. The $s(n)$ in the second part is a control variable which represents the saving rate. $\left(1-a_{1} T_{\mathrm{AT}}(i) - a_{2} T_{\mathrm{AT}}(i)^{2} \right)$ and $\left(1-\theta_{1}(i) \mu(i)^{\theta_{2}}\right)$ are the proportion of the loss of capital accumulation due to the temperature increasing and contributions to reducing carbon emission correspondingly.

\subsubsection{Environmental Dynamics}
\paragraph{Carbon Mass}
\begin{equation}
    \begin{aligned}
    M(i+1) &=\Phi_{M} M(i)+B_{M} E(i)\\
    \text{where}\\
    E(i) &= \sigma(i)(1-\mu(i)) A(i) K(i)^{\gamma} L(i)^{1-\gamma}+E_{\mathrm{Land}}(i)\\
    M &\doteq\left[\begin{array}{lll}M_{\mathrm{AT}} & M_{\mathrm{UP}} & M_{\mathrm{LO}}\end{array}\right]^{\top} \in \mathbb{R}^{3}\\
    \Phi_{M} &\doteq\left[\begin{array}{ccc}\zeta_{11} & \zeta_{12} & 0 \\ \zeta_{21} & \zeta_{22} & \zeta_{23} \\ 0 & \zeta_{32} & \zeta_{33}\end{array}\right]\\
    B_{M} &\doteq\left[\begin{array}{c}\xi_{2} \\ 0 \\ 0\end{array}\right]
    \end{aligned}
\end{equation}
This dynamic describe a three-reservoir model of the global carbon cycle, in which the $M_{AT}$ describes the average mass of carbon in the atmosphere, $M_{UP}$, the average mass of carbon in the upper ocean and $M_{LO}$ the average mass of carbon in the deep or lower ocean. $\Phi_{M}$ is the Markov transition matrix describing how carbon transfer between different reservoirs. $B_{M}$ describes how the weight of carbon emission affects the carbon accumulation in the reservoirs. To conclude, the three-reservoir model can be described in figure \ref{fig:three-reservoir}.

\begin{figure}
    \centering
    \includegraphics[width=8cm]{figures/three-reservoir.png}
    \caption{the three-reservoir model}
    \label{fig:three-reservoir}
\end{figure}

\paragraph{Global Temperature}
\begin{equation}
    \begin{aligned}
    T(i+1) &=\Phi_{T} T(i)+B_{T}F(i)\\
    \text{where}\\
    T &\doteq\left[\begin{array}{lll}T_{\mathrm{AT}}& T_{\mathrm{LO}}\end{array}\right]^{\top} \in \mathbb{R}^{2}\\
    F(i)&=F_{2 \times} \log _{2}\left(\frac{M_{\mathrm{AT}}(i)}{M_{\mathrm{AT}, 1750}}\right)\\
    \Phi_{T} &\doteq\left[\begin{array}{ll}\phi_{11} & \phi_{12} \\ \phi_{21} & \phi_{22}\end{array}\right]\\
    B_{T} &\doteq\left[\begin{array}{l}\xi_{1} \\ 0\end{array}\right]
    \end{aligned}
\end{equation}

Similar to the carbon mass dynamic, there are two layers in the energy balance model. The $T_{AT}$ the combined average temperature in atmosphere, land surface, and upper ocean (simply referred to as the atmospheric layer in what follows) and the $T_{LO}$ is the lower ocean. $\Phi_{T}$ is the Markov transition matrix describing how temperature transfer between different layers. $B_{T}$ describes how the weight of the way that carbon accumulation contributing to the temperature raises. To conclude, the energy balance model is shown in figure \ref{fig:energy-model}

\begin{figure}
    \centering
    \includegraphics[width=4cm]{figures/energy-model.png}
    \caption{the energy-model}
    \label{fig:energy-model}
\end{figure}





% \begin{enumerate}
%     \item trade : armington, etc.
%     \item tariffs : import tariffs, redistribution of income
% \end{enumerate}


% \srp{Brief description of the DICE model and put the equations as implemented in the simulator in the Appendix}

% \srp{Describe RICE model: how the above DICE model is adapted to take into account various regions} 

% \srp{Adding Trade and tariffs to this model.}


==> src_AAAI/model.tex <==
%!TEX root = main.tex

\section{The \SimulationName{} Integrated Assessment Model}
\label{sec:ABM}

\begin{figure*}
    \centering
    \includegraphics[width=0.75\linewidth]{figures/sim-overview.png}
    \caption{\textbf{Schematic overview of the observables, actions, and components in \SimulationName{}.} 
    % 
    Each region (agent) uses a policy model to negotiate and make climate, economic, and trade decisions. 
    % 
    For clarity, we show the flow of information and actions for a single agent only.
    % 
    The details of the negotiation protocol are up to users to implement.
    % 
    At a high-level, at each timestep, each policy first receives an observation of the negotiation and world state and decides how to negotiate.
    % 
    Negotiation may proceed for several iterations (at the same timestep).
    % 
    The outcome of all negotiations are agreements (or lack thereof), which may be between two or more agents. 
    % 
    In particular, an agreement may influence the remaining actions that an agent can take in the climate and economic domains.
    % 
    For the same timestep, each agent then makes decisions with respect to the climate, economy, and trade. 
    % 
    }
    \label{fig:simulation-schema}
\end{figure*}


We introduce \SimulationName{}, an IAM that augments RICE with a framework for negotiation protocols, and further includes international trade and tariffs, as in \cite{lessmann2009effects}.
% 
Each agent represents a (fictitious) region or nation and chooses its levels of capital investment, mitigation effort, and international trades and tariffs, for each time step (e.g., every 5 years).
% 
\SimulationName{} can be configured with an arbitrary number of agents and shares economic and social characteristics with the real world.


\textbf{The structural parameters of the public version of \SimulationName{} have been fitted to real data.
% 
However, the public version is not a one-to-one, identical representation of the real world. 
% 
The individual agents do not represent real-world nations.
}

\SimulationName{} is designed to be easily extendable and modular. 
%  
In particular, \SimulationName{} provides a framework to implement negotiation protocols as well as learning algorithms (e.g., reinforcement learning agents) to enable designing negotiation protocols and study their effects on global cooperation.


\paragraph{Formal definitions.}
% 
The equations in the \SimulationName{} dynamics largely follow the RICE model and are listed in Appendix \ref{sec:params-and-vars}, see also \cite{kellett2019feedback} for more details.
% 
See Appendix \ref{sec:params-and-vars} for an overview of all state variables (Table \ref{tab:world_state_var}, action variables (Table \ref{tab:agent_action_var}), structural parameters (Table \ref{tab:global_constants}), and regional parameter (Table \ref{tab:agent_charact}).
% 
We set the values of the parameters using the data and procedure in \cite{kellett2019feedback} and \cite{nordhaus2007review}, while others are calibrated using historical time series data (see the Appendix for more details).


In \SimulationName{}, there are $\numRegions$ regions, where each region is modeled as an independent decision-making agent.
% 
These regions are fictitious.
% 
Regions interact with each other and the environment through their actions: setting a savings rate, mitigation rate, trades and tariffs, and negotiation actions.


\paragraph{\SimulationName{} base dynamics.}
% 
The simulation has two main components: \emph{negotiation} and \emph{climate-economic activity}, see Figure~\ref{fig:simulation-schema}.
% 
The activity component is the core component that simulates the physical actions of the agents and the resulting evolution of the environment.
% 
The negotiation component is an additional component that simulates communication between the regions that is necessary in forming agreements between the regions. 
% 
In addition, agreements may adjust the available actions for each region during the activity stage.


Each simulation episode consists of $\numEpisodeSteps$ steps, each step representing $\numStepPeriod$ years (e.g, $\numStepPeriod=5$).
% 
Thus, the simulation spans a period of $\numEpisodeSteps \times \numStepPeriod$ simulation-years.
% 
At every step, the simulation goes through the negotiation stages and agreements are formed within the regions.
% 
The simulation then enters the activity stage where each region takes actions that comply with the agreements formed during the negotiation stages.


\paragraph{Climate-economic activity.}
% 
The activity component of the simulation includes the following actions: the region's mitigation rates, and savings rates for capital investment, the tariffs imposed by this region on other regions, its maximum export limits, and import bids to other regions (see Table~\ref{tab:agent_action_var}).

The activity component simulates the effect of the activity stage actions on the world climate and the economy.
% 
The \emph{state of the world} is characterized by global variables such as the concentration of carbon dioxide in the Earth's atmosphere, and the average global temperature, as well as region specific variables such as population, capital, technology level, carbon intensity of economic activity, and balance of trade (see Table~\ref{tab:world_state_var}).
% 
% These activity stage actions govern the evolution of the environment.
% % 
% These actions include savings rate, mitigation rate, international tariffs, export limits, and import bids, see Table~\ref{tab:agent_action_var}. 
% % 
% For example, the savings rate determines the fraction of output production over the next 5 years that this region wants to invest in its capital.


At every step, the simulator does the following (additional details provided in Section~\ref{sec:dynamics}): 
%
The gross output production for each region is computed based on the state of the region, in particular, its capital investment, labor (or population), and technology factor. 
% 
The net economic output is the gross output production reduced by climate damages from rising global temperature, and the cost of efforts towards mitigation by this region.
% 
The region consumes domestic goods equal to the quantity of the net economic output that is left after capital investment and export.
% 
It also consumes foreign goods from imports.
% 
The consumption utility for each region from consuming domestic and foreign goods is computed using the Armington elasticity assumption that has become standard in international computable general equilibrium models \cite{armington1969theory}.
% 
This gives the \emph{reward} corresponding to each region in every step. 
%

In economic terms, variables such as capital, balance of trade, carbon mass, and global temperature depend on the agents' actions and are called \emph{endogenous} variables.
% 
On the other hand, variables such as population, technology level, carbon intensity of economic activity are called \emph{exogenous}, i.e., their values do not depend on the agent actions.
% 
Note that the values of endogenous variables can vary across steps in a predetermined manner.


\paragraph{Negotiation.}
% 
The negotiation component can include different stages of communication and the rules to form agreements between the regions.
% 
Note that the simulator can work with an empty negotiation component, and indeed these provide important baselines for performance evaluation.
% 
\emph{The focus of this competition is to test different negotiation protocols that affect the actions during the activity stage and lead to socially better outcomes.}


In the base implementation of \SimulationName{}, we allow the negotiated agreements to control the range of actions allowed for the regions.
% 
% For example, an agreement could state that a given region should implement a minimum of $20\%$ mitigation rate.
%
The effect of an agreement can then be encoded in the form of \emph{action masks} that control the allowed action space during the activity stage.
% 
For example, an agreement could state that a given region should implement a minimum of $20\%$ mitigation rate.
% if an agent promises to save at least $10\%$, 
Then the action mask only allows setting mitigation rates above that level for this region.
% 
Hence, it is important to ensure that the negotiation protocol provides each region a way to reject any agreement that restricts its actions.
%
For example, it shouldn't happen that a certain region is forced to implement a mitigation rate that it did not agree upon.
% 
Alternatively, an implementation can include agent observations that allow regions to check if the agreements were followed and learn to punish the regions that did not comply with them.
%
Such an implementation would be more realistic  as compared to an implementation based on action masks because they do not assume any agreement enforcing entity.
%




% Depending on the actions by all the regions and the evolution of the environment, each region consumes certain domestic goods and certain foreign goods from other countries.


%\srp{%
%Explain that the provided simulation takes care of the activity stage and integration with the agreements from negotiation stages. 
%Explain what the agreements look like in our simulation.
%The users can implement the negotiation protocol of their choice in the negotiation block.
%Finally, the entire simulation is run by modeling the regions as RL agents.
%}



% \srp{Explain how RL works in brief.}


% \srp{Explain observations to RL agents. World related observations are fixed. Negotiation related observations can be modified.}

% \srp{Explain actions to RL agents. Activity actions are fixed. Negotiation related actions can be modified.}

% \srp{Explain reward to RL agents.}


% Agent specific characteristics such as initial population, capital, technology level, carbon intensity of economic activity, and their growth rates, Armington elasticities, and long term welfare discount rates are given in table~\ref{tab:agent_charact}.

% \srp{Describe the metrics that the simulator outputs. Evaluation for competition based on these metrics.}



\paragraph{Customization.}

% 
The simulation code is structured so that custom negotiation protocols can be implemented as part of the negotiation component.
%
An implementation may add agent observations and actions corresponding to the proposed negotiation protocol, 
and rules to generate the corresponding agreements.
%
Notice that the agents can have access to these additional observations even during the activity stage.
%
These observations are useful in letting the agents adopt policies in response to the negotiations and agreements.
%
For example, they can learn to punish agents that do not comply with the agreements. 
%
Besides, by using action masking, the simulation can ensure that the agreements are followed (we can also have mix where some agreements are enforced using action masking and some others are non-enforceable).
%
Thus, the simulation code provides complete freedom in implementing any negotiation protocol of choice provided the corresponding agreements are appropriately connected to the activity stage action through additional observations or action masks.
%
Further implementation details are in Appendix \ref{sec:engineering-details}.

% The jury will include these practicality criteria while evaluating the solutions in track II of the competition.
% %
% \srp{Include description of the three tracks in the document.}




% \srp{Describe the primary actions available for each agent, namely, mitigation rate, savings rate, import bids, export limits, tariffs}

% \srp{Describe agents outcomes such as consumption and preferences on these outcomes such as aggregate discounted welfare.}

% \srp{Mention that additional state variables, agent actions, rewards will be added based on the negotiation protocol. See sec. \ref{sec:model_negotiation_framework}}



\section{The Activity Component: Climate, Economics, Trade, and Tariffs}
\label{sec:dynamics}
% 
The \SimulationName{} simulation builds on the RICE model \cite{nordhaus2015climate}, a multi-region climate-economic simulation, by adding negotiation protocols, international trade, and support for strategic agents. 
% 
\SimulationName{} has $\numRegions$ agents which each represent a region in the world, or a group of (fictitious) countries that are assumed to make decisions as a single entity.
% 
To maintain realism, we calibrate the structural parameters and establish a reasonable range of agent-specific parameters using data from the World Bank API \cite{wbapi}.
% 
The full flow of the activity component is shown in Algorithm \ref{alg:cap} in Appendix \ref{sec:rice-dynamics-details}.


\subsection{Climate and Economic Dynamics}
% 
We now describe the RICE dynamics that govern the evolution of the world state from time $\idstep$ to $\idstep+1$ for the different regions. 
% 
Note that variables without an agent index are global quantities.

% We now describe these equations in more detail.

% \stz{Tianyu: Can you explain how you chose $\theta_1$, $\theta_2$? Are those global or regional quantities?}
% 
% \srp{There seems to be a typo in equation (4). Should it be $\sigma_{i,t}$? What is the relation between $\theta_{1,t}$ and $\theta_1(i)$?} stz: fixed this

% 
% For clarity, we will omit the region subscript $\idxi$ below. 
% % 
% All the regions are assumed to follow the same dynamic equations with region specific parameters.


% \srp{Would it be possible to give a short description of the equations and move the details to the appendix? This is because I don't think the competitor need all the details below as long as they have a rough idea about the dependence of parameters on each other. For example, temperature depends on carbon mass which depends on emissions which depends on production, etc.}

% \subsubsection{Environmental Dynamics}

\paragraph{Carbon mass.}
% 
The total carbon mass in the climate system is given by:
% 
\eq{
\xcarbonmass_{\idstep+1} &=\Phi_{M} \xcarbonmass_{\idstep}+B_{M} \sum_{i}\xemission_{\idxi, \idstep}, \\
\xemission_{\idxi, \idstep} &= \xemission^{\textrm{Land}}_{\idstep}+ \xcarbonintensity_{\idxi, \idstep} \xtechnology_{\idxi, \idstep} (1-\mu_{\idxi, \idstep}) \xproduction_{\idxi, \idstep} \label{eq:sigma-t}, \\
% 
\xcarbonmass_{\idstep} &\doteq\left[\begin{array}{lll}\xcarbonmass^{\textrm{AT}}_{\idstep} & \xcarbonmass^{\mathrm{UP}}_{\idstep} & \xcarbonmass^{\mathrm{LO}}_{\idstep}\end{array}\right]^{\top} \in \mathbb{R}^{3}, \\
% 
\Phi_{M} &\doteq\left[\begin{array}{ccc}\zeta_{11} & \zeta_{12} & 0 \\
\zeta_{21} & \zeta_{22} & \zeta_{23} \\ 0 & \zeta_{32} & \zeta_{33}\end{array}\right], \\
B_{M} &\doteq\left[\begin{array}{c}\xi_{2} \\ 0 \\ 0\end{array}\right].
}
% 
This describes a three-reservoir model of the global carbon cycle, in which $M_{AT}$ describes the average mass of carbon in the atmosphere, $M_{UP}$ is the average mass of carbon in the upper ocean, and $M_{LO}$ the average mass of carbon in the deep or lower ocean, see Figure \ref{fig:three-reservoir}. 
% 
$\Phi_{M}$ is the Markov transition matrix describing how carbon transfer between different reservoirs. 
% 
$B_{M}$ describes how the weight of carbon emission affects the carbon accumulation in the reservoirs.

\begin{figure}
    \centering
    \includegraphics[width=8cm]{figures/three-reservoir.png}
    \caption{
    \textbf{The three-reservoir carbon mass model.}
    }
    \label{fig:three-reservoir}
\end{figure}

\paragraph{Global temperature.}
% 
Ultimately, increasing carbon mass leads to rising temperatures:
% 
\eq{
    \xtemperature_{\idstep+1} &=\Phi_{T} \xtemperature_{\idstep}+B_{T}\xforcing_{\idstep}, \\
    \xtemperature_{t} &\doteq\left[\begin{array}{lll}\xtemperature^{\textrm{AT}}_{t}& \xtemperature^{\textrm{LO}}_{t}\end{array}\right]^{\top} \in \mathbb{R}^{2}, \\
    \xforcing_{\idstep} &= F_{2 \times} \log _{2}\left(\frac{\xcarbonmass^{\textrm{AT}}_\idstep}{\xcarbonmass^{\textrm{AT}, 1750}}\right), \\
    \Phi_{T} &\doteq\left[\begin{array}{ll}\phi_{11} & \phi_{12} \\ \phi_{21} & \phi_{22}\end{array}\right], \\
    B_{T} &\doteq\left[\begin{array}{l}\xi_{1} \\ 0\end{array}\right].
}

Similar to the carbon mass dynamic, there are two layers in the energy balance model, see Figure \ref{fig:energy-model}.
% 
$T_{AT}$ is the combined average temperature in atmosphere, land surface, and upper ocean (simply referred to as the ``atmospheric layer'' hereafter). 
% 
$T_{LO}$ is the temperature in the lower ocean. 
% 
$\Phi_{T}$ is the Markov transition matrix describing how heat transfers between different layers. 
% 
$B_{T}$ describes how carbon mass contributes to the temperature increases. 

% \paragraph{Damage Function}
% The climate damage function represent economic damages as a function of climate indicator inputs. 
% In our case, it is the increment of the atmosphere temperature $\xtemperature_{\idstep}^{\textrm{AT}}$. In equation \ref{eq:rice:capital}, following the form of damage function from \cite{nordhaus2015climate}, the form is 
% \begin{equation} \label{eq:rice:damage}
%     {1-a_{1} \xtemperature^{\textrm{AT}}_{\idstep} - a_{2}\xtemperature^{\textrm{AT}}_{\idstep}}^{2}
% \end{equation}


% \subsubsection{Economic Dynamics}
 
\paragraph{Output production.}
% 
The production in a region is given by the \emph{total factor productivity (TFP)} \cite{Comin2010} formula:
% 
\eq{ \tag{\ref{eq:rice:production}}
\xproduction_{\idxi, \idstep} = \xtechnology_{\idxi, \idstep}\xcapital_{\idxi, \idstep}^{\gamma}\xpopulation_{\idxi, \idstep}^{1-\gamma}.
}
% 
Production depends on three factors: total factor productivity (``technology'') $\xtechnology_{\idstep}$, capital $\xcapital_{\idstep}$, and labor $\xpopulation_{\idstep}$. 
% 
This production function is common in the economic literature and used in the DICE/RICE models. 
% 
The capital elasticity $\gamma \in [0,1]$ explains the different levels of contribution of capital and labor. 


\paragraph{Population.}
% 
The number of people in a region, denoted $\xpopulation_{\idstep}$ grows as:
% 
\begin{equation} \tag{\ref{eq:rice:population}}
\xpopulation_{\idxi, \idstep+1} =\xpopulation_{\idxi, \idstep}\brck{ \frac{1+\xpopulation_{a; \idxi}}{1+\xpopulation_{\idxi, \idstep}} }^{l_{g; \idxi}}.
\end{equation}

There are two parameters $L_{A;\idxi}$ and $l_{g; \idxi}$. $L_{a; \idxi}$ represents the convergence population of region $\idxi$ and $l_{g; \idxi}$ shows how fast the population $L_{\idxi, \idstep}$ converge to $L_{a; \idxi}$. 
% 
Please refer to the Appendix for a more detailed analysis and the calibration procedure. 


\paragraph{Level of technology.}
% 
The technology factor $A_{\idstep}$ describes how efficient production is, i.e., how many units of output a region achieves given fixed capital and labor:
% 
% A_i * (np.exp(0.0033) + g_A * math.exp(-delta_A * Delta * (ii - 1)))
\eq{ \tag{\ref{eq:rice:technology}}
\xtechnology_{\idxi, \idstep+1} &= (e^\eta + g_{A;\idxi} e^{-\delta_{A;\idxi} \Delta(\idstep-1)} ) \xtechnology_{\idxi, \idstep}.
}

Here, $\eta$ represents the long-term growth of economics which is usually larger than 0,
% 
$g_A$ represents the short-term part of economics growth,
% 
and $\delta_A$ represents the speed of decay of short-term growth factor.
% 
$\Delta$ is the time difference between steps. 
% 
We use $\eta = 0.33\%$ as in \cite{RePEc:spr:climat:v:148:y:2018:i:4:d:10.1007_s10584-018-2218-y}.



\paragraph{Capital.}
% 
The amount of capital evolves as:
% 
\eq{ 
\Phi_{K} &\doteq \left(1-\delta_{K}\right)^{\Delta}, \\
% 
\xcapital_{\idxi, \idstep+1} &=\Phi_{K, \idxi} \xcapital_{\idxi, \idstep}+\Delta\brck{1-a_{1} \xtemperature^{\textrm{AT}}_{\idstep} - a_{2} \brck{\xtemperature^{\textrm{AT}}_{\idstep}}^{2} } \\
&\times \left(1-\theta_{1; \idxi,\idstep} \mu_{\idxi, \idstep}^{\theta_{2}}\right) \xproduction_{\idxi, \idstep} \xsavings_{\idxi, \idstep}.
}
The evolution of the capital comes from two parts. 
% 
The first part is capital inherited from the previous period with depreciation. 
% 
In the second part, $\xsavings_{\idstep}$ is a control variable which represents the investment/savings rate (as a fraction of production). 
% 
That is, as a base amount, the economy invests/saves a total of $\xproduction_{\idxi,\idstep} \xsavings_{\idxi, \idstep}$ 
which yields new capital.
% 
This base amount is further modified by 2 multipliers: the damage function and mitigation/abatement costs, which are discussed below.

% \subsubsection{Climate-Economic Dynamics}

\paragraph{Damage function.}
% 
The climate damage function represents the economic damage due to climate change, e.g., increases in the atmosphere temperature $\xtemperature_{\idstep}^{\textrm{AT}}$. 
% 
That is, in Equation \ref{eq:rice:capital}, the fraction of new capital is modified by the damage function
% 
\eq{\label{eq:damage-function}
1-a_{1} \xtemperature^{\textrm{AT}}_{\idstep} - a_{2} \brck{\xtemperature^{\textrm{AT}}_{\idstep}}^{2},
%
} 
following \cite{nordhaus2015climate}.
% 
That is, higher temperatures lead to less new capital.
% 
Similarly, $1-\theta_{1;\idxi, \idstep} \mu_{\idstep}^{\theta_{2}}$ is the fraction of new capital after taking into account carbon emission mitigation.
% 
Mitigating carbon emissions more (higher $\mu_{\idstep}$) means (dirty) production needs to be lowered, hence yields less new capital.


\paragraph{Mitigation (abatement) cost.}
% 
Following \cite{kellett2019feedback}, for a mitigation rate $ \mu_{\idxi, \idstep}$, the mitigation cost is 
\eq{\label{eq:mitigation-cost}
\theta_{1; \idxi,\idstep} \mu_{\idxi, \idstep}^{\theta_{2}}\xproduction_{\idxi,\idstep} \xsavings_{\idxi, \idstep},} 
% 
where $\theta_{1; \idxi, \idstep}$ is given by Equation \ref{eq:rice:cost_of_mitigation_efforts}.
% 
This represents the loss in capital growth due to a fraction of production being used for mitigation.
% 
% That is, more mitigation lowers the amount of new capital created. 


\paragraph{Carbon intensity of economic activity.}
% 
A critical part of the model is the interaction between the climate and economic parts. 
% 
Specifically, the RICE model describes how production leads to carbon emissions:
% 
\eq{
\xemission^{\textrm{Land}}_{\idstep}&=\xemission_{L0} \cdot\left(1-\delta_{EL}\right)^{t-1}, \\
\xemission_{\idxi, \idstep} &= \xemission^{\textrm{Land}}_{\idstep}+ \xcarbonintensity_{\idxi, \idstep} \xtechnology_{\idxi, \idstep} (1-\mu_{\idxi, \idstep}) \xproduction_{\idxi, \idstep} \\
\xcarbonintensity_{\idxi, \idstep+1} &=\xcarbonintensity_{\idxi, \idstep} e^ {-g_{\xcarbonintensity; \idxi}\brck{1-\delta_{\xcarbonintensity; \idxi}}^{\Delta(\idstep-1)} \Delta}.
}
% 
Here $\xemission^{\textrm{land}}_{\idstep}$ is the carbon emission due to (changes in) land use, 
% 
$\xemission_{L0}$ is the carbon emission in the base year, 
% 
and $\delta_{EL}$ is the speed of decrease of changes in land use.
% 
The rates $0 < \delta_{EL} < 1$, $0 <\delta_{L0} < 1$ are free parameters. 
% 
Due to a lack of data, $\xemission^{\textrm{land}}_{\idstep}$ is set to be the same for each region.


$\xemission_{\idxi, \idstep}$ is the total carbon emission, $\xemission_{t}^{\textrm{land}}$ is emission from natural sources, while $\xemission_{\idxi, \idstep} - \xemission_{t}^{\textrm{land}}$ is emission caused by economic activity.
% 
$\xcarbonintensity_{\idxi, \idstep}\xtechnology_{\idxi,\idstep}$ is the effective carbon intensity of economic activity: a higher technology factor lead to higher emissions, but can be modulated by lower $\xcarbonintensity$ (which can be thought of as the degree of ``clean'' production).
% 
$\mu_{idxi, \idstep} \in [0, 1]$ is a control variable called the abatement (ratio), which represents the proportion of the economics contributing to reducing carbon emission. 
% 
Furthermore, we have 2 parameters $g_{\xcarbonintensity}$ and $\delta_{\xcarbonintensity}$ that are fitted to data. 
% 
$g_{\xcarbonintensity}$ is the rate of decrease in carbon emissions.


% \paragraph{Damage function.}
% % 
% The climate damage function represents the economic damage due to climate change, e.g., increases in the atmosphere temperature $\xtemperature_{\idstep}^{\textrm{AT}}$. 
% % 
% In Equation \ref{eq:rice:capital}, following \cite{nordhaus2015climate},
% the fraction of new capital is $\left(1-a_{1} \xtemperature^{\textrm{AT}}_{\idstep} - a_{2} \brck{\xtemperature^{\textrm{AT}}_{\idstep}}^{2} \right)$.
% %
% That is, higher temperatures lead to less new capital.
% % 
% Similarly, $\left(1-\theta_{1;\idxi, \idstep} \mu_{\idstep}^{\theta_{2}}\right)$ is the fraction of new capital after taking into account carbon emission mitigation.
% % 
% Mitigating carbon emissions more (higher $\mu_{\idstep}$) means (dirty) production needs to be lowered, hence yields less new capital.





% \paragraph{Mitigation (abatement) cost.}
% % 
% Following \cite{kellett2019feedback}, for a mitigation rate $ \mu_{\idxi, \idstep}$, the mitigation cost is $\theta_{1; \idxi,\idstep} \mu_{\idxi, \idstep}^{\theta_{2}}\xproduction_{\idxi,\idstep} \xsavings_{\idxi, \idstep}$ where $\theta_{1; \idxi, \idstep}$ is given by Equation \ref{eq:rice:cost_of_mitigation_efforts}.
% % 
% This represents the loss in capital growth due to a fraction of production being used for mitigation.
% % 
% % That is, more mitigation lowers the amount of new capital created.         





    
\begin{figure}
    \centering
    \includegraphics[width=4cm]{figures/energy-model.png}
    \caption{\textbf{The two-reservoir temperature model.}}
    \label{fig:energy-model}
\end{figure}

\comment{
Similarly, the technology level and the carbon intensity of economic activity are generated by the following equations.
\eq{
A_{\idstep+1} &=(\exp\eta+g_{A} \exp \left(-\delta_{A} \numStepPeriod(\idstep-1)\right))A_{\idstep} \\
\xcarbonintensity_{\idstep+1} &=\xcarbonintensity_{\idstep} \exp \left(-g_{\xcarbonintensity}\left(1-\delta_{\xcarbonintensity}\right)^{\numStepPeriod(\idstep-1)} \numStepPeriod\right)
}
The technology level plays the role of total factor productivity in the production function (see equation ??).
The carbon intensity of economic activity gives the level of emissions based on production and mitigation activities (see equation ??).
See Appendix for further details on the meanings of the different parameters in these equations and our calibration process using data from the world bank.


\srp{Include plots of these three variables as a function of time for a sample region}

The gross production output for each region is given by the product of three terms: the total factor productivity (technology level) $\xtechnology$, capital $\xcapital$, and labor $\xpopulation$ (which is approximated by the region's population). 
The capital elasticity $\gamma \in [0,1]$ explains the different contribution level of capital and labor.
\begin{equation}
    \xproduction_{\idxi, \idstep} = \xtechnology_{\idxi, \idstep}\xcapital\xpopulation_{\idxi, \idstep}^{\gamma}\xpopulation_{\idxi, \idstep}^{1-\gamma}
\end{equation}

The net economic output $\xnetoutput$, is gross output production reduced by two factors: climate damages from rising atmospheric temperature, and cost of efforts towards mitigation.
\begin{equation}
    \xnetoutput_{\idxi, \idstep} = \left(1-a_{1} \xtemperatur\xemission^{\textrm{AT}}_{\idstep} - a_{2} \xtemperatur\xemission^{\textrm{AT}}_{\idstep}^{2} \right)\left(1-\theta_{1}_{\idstep} \xmitigation_{\idxi, \idstep}^{\theta_{2}}\right)
    \xproduction_{\idxi, \idstep}
\end{equation}

The savings to be invested in the region's capital is given by
\begin{equation}
    \xinvest_{\idxi, \idxi}_{\idstep} = \xnetoutput_{\idxi, \idstep} \xsavings_\idstep_{\idstep}.
\end{equation}


The contribution to the total emissions by region $\idxi$ is given by
\begin{equation}
    \xemission_{\idxi, \idstep} = \xcarbonintensity_{\idxi, \idstep}(1-\xmitigation_{\idxi, \idstep}) \xproduction_{\idxi, \idstep}
\end{equation}

Thus the total emissions by all regions at step $\idstep$ is given by
\begin{equation}
    \xemission_{\idstep} = \sum_\idxi \xemission_{\idxi, \idstep}.
\end{equation}

The carbon mass dynamics is given by
\begin{equation}
    \xcarbonmass_{\idstep+1} =\Phi_{M} \xcarbonmass_{\idstep}+B_{M}\left(\xemission_{\idstep} +\xemission_{\mathrm{Land}}_{\idstep}\right)
\end{equation}

% \srp{@Tianyu Please confirm if the emission dynamics are correct here. Are the land emissions specific to region or independent of regions? Do they change with time?}

The global temperature changes as follows:
\begin{equation}
    \xtemperature_{\idstep+1} =\Phi_{T} \xtemperature_{\idstep}+B_{T}\left(F_{2 \times} \log _{2}\left(\frac{\xcarbonmass_{\mathrm{AT}}_{\idstep}}{\xcarbonmass_{\mathrm{AT}, 1750}}\right)+F^{\textrm{EX}}_{\idstep}\right)
\end{equation}
}

\subsection{Trade}

% \srp{@Andrew please edit this section.}


We now describe the international trade dynamics and the resulting regional consumption and utilities.
Regions trade by exporting their own consumption goods and importing other regions' consumption goods at a fixed unit price\footnote{More generally, prices should be dynamic, but the current implementation does not support this.}.

% Since each region produces its own distinct consumption good, total trade flow during time $t$ can be represented by a matrix $\xtransfermatrix_{\idstep}$ where the element $\xtransfer_{\idxi,\idxj,\idstep} \geq 0$ represents the transfer of goods from region $\idxj$ to region $\idxi$ at time $\idstep$, the row vector $ \Vec{\xtransfer}_i = [\xtransfer_{\idxi,1}, ..., \xtransfer_{\idxi,\idxk}]$ represents the transfer of goods to region $\idxi$ from all regions $\idxj$ and the vector 
% $\Vec{x}_\idxi = [\xtransfer_{1, \idxi}, ... , \xtransfer_{\idxk, \idxi}]$ represents the exports from region $\idxi$ to all regions $\idxj$.
% For all regions, $\xtransfer_{\idxi, \idxi} = 0$.

\paragraph{Agent actions.}
% To obtain $\xtransfermatrix_{\idstep}$, each
Each region $\idxi$ at time $t$ must first specify a desired basket of consumption goods $ \bm{\ximportbid_{\idxi,t}} = [\ximportbid_{\idxi,1,t}, ..., \ximportbid_{\idxi, \idxk,t}]$ that they are willing to import from the other regions.
These desired imports form a matrix of \textit{bids} $\ximportbidmatrix_{\idstep}$ such that the import bid by region $\idxi$ for goods from $\idxj$ at time $\idstep$ is $\ximportbid_{\idxi,\idxj,\idstep} \geq 0$, i.e., the amount of goods region $\idxi$ is willing to import from region $\idxj$ at time $\idstep$ is $\ximportbid_{\idxi,\idxj,\idstep}$.

Regions also set an upper bound $\xexportlimit_{\idxi, \idstep} \in [0,1]$ on the proportion of their own consumption goods that they are willing to export.


% 
% If the trade balance of a region exceed its gross output at a given period, then this region can no longer import goods from other regions and must contribute revenue from imports toward its trade balance.



\paragraph{Tariffs.}
% 
Regions can also choose to impose import tariffs on other regions.
We denote an import tariff imposed by region $\idxi$ on a region $\idxj$ by $\xtariff_{\idxi,\idxj,\idstep} \in [0,1]$.
% 
If region $\idxi$ imposes an import tariff $\xtariff_{\idxi,\idxj,\idstep} \in [0,1]$ on region $\idxj$, region $\idxi$ consumes 
% 
\begin{equation} \label{eq:trade:tariff_goods}
    \xconsumption_{\idxi,\idxj,\idstep} = \xgoodstraded_{\idxi,\idxj,\idstep} (1 - \xtariff_{\idxi,\idxj,\idstep}),
\end{equation}
% Thus, if $\ximportbid_{\idxi,\idxj,\idstep}$ goods are exported from region $\idxj$ to region $\idxi$ then region $\idxi$ makes a payment of $\ximportbid_{\idxi,\idxj,\idstep}$ dollars to region $\idxj$.

% Since, the price of international trade is fixed, to avoid excessive total exports from a region, we let each region set a maximum limit on its export 
% \begin{equation}
%     \xmaxexportlimit_{\idxi, \idstep} \leq \xnetoutput_{\idxi, \idxi}_{\idstep} - \xinvest_{\idxi, \idstep}.
% \end{equation}
% This denotes the maximum amount of domestic production this region is willing to export at a unit price.

and $\tau_{\idxi, \idxj, \idstep}x_{\idxi,\idxj,\idstep}$ is added to a reserve fund specific to that region.
% 
\paragraph{Consumption.}

Consumption of domestic goods $\xconsumption_{i,i,t}$ is determined according to gross output, the savings rate and exports:

\begin{equation}
    \label{eq:consumption_domestic}
    \xconsumption_{i,i,t} = (1 - \xsavings_{i,t})\xgrossoutput_{i,t} - \sum_{\idxj \neq \idxi} \xgoodstraded_{\idxj,\idxi,t}.
\end{equation}

The aggregated consumption $C_{\idxi, \idstep}$ at time $t$ for region $\idxi$ is given by the Armington elasticity model~\cite{lessmann2009effects}) as follows:
% 
\begin{equation} \label{eq:agg_consumption}
    C_{\idxi, \idstep} = \brck{  \psi^{dom}(\xconsumption_{\idxi, \idxi, \idstep})^\lambda +  \sum_{j\neq i} \psi^{for} (\xconsumption_{\idxi, \idxj, \idstep})^\lambda  }^{\fr{1}{\lambda}}.
\end{equation}


% If the balance of trade is negative then the region has a foreign debt.
% To avoid regions from accumulating foreign debt we restrict the country from importing goods if its foreign debt becomes higher than $10\%$ of its capital.
% Thus, if at step $\idstep$, $\xtradebalance_{\idxi, \idstep} < - 0.1\xcapital\xpopulation_{\idstep}$, then $\ximportbid_{\idxi, \idxj} = 0$ for all $\idxj$.

% \srp{Complete the algorithm to match with latest code version}


% \srp{@Andrew Please check if the trades and tariffs logic seems okay. 
% I believe currently the tariff revenue is burnt or added to trade deficit. 
% I think we should change it and add to capital investment. Another change is the condition on limiting foreign debt. 
% I think current implementation absolves a region of any foreign debt if it is not cleared by borrowing from production in the next step. 
% I don't like the idea of forcing a region to use its production to clear its foreign debt and certainly not of absolving it if it fails to clear its debt. 
% Instead I think it is more natural that the other regions stop exporting goods to this country if its foreign debt is large compared to its capital.
% Let me know what you think?}

















